Time Fairness in Online Knapsack Problems

The online knapsack problem is a classic problem in the field of online algorithms. Its canonical version asks how to pack items of different values and weights arriving online into a capacity-limited knapsack so as to maximize the total value of the admitted items. Although optimal competitive algorithms are known for this problem, they may be fundamentally unfair, i.e., individual items may be treated inequitably in different ways. We formalize a practically-relevant notion of time fairness which effectively models a trade off between static and dynamic pricing in a motivating application such as cloud resource allocation, and show that existing algorithms perform poorly under this metric. We propose a parameterized deterministic algorithm where the parameter precisely captures the Pareto-optimal trade-off between fairness (static pricing) and competitiveness (dynamic pricing). We show that randomization is theoretically powerful enough to be simultaneously competitive and fair; however, it does not work well in experiments. To further improve the trade-off between fairness and competitiveness, we develop a nearly-optimal learning-augmented algorithm which is fair, consistent, and robust (competitive), showing substantial performance improvements in numerical experiments.

==> 0frontmatter.tex <==






\makeatletter
\newcommand{\algmargin}{\the\ALG@thistlm}
\makeatother
\newlength{\whilewidth}
\settowidth{\whilewidth}{\algorithmicwhile\ }
\algdef{SE}[parWHILE]{parWhile}{EndparWhile}[1]
{\parbox[t]{\dimexpr\linewidth-\algmargin}{%
		\hangindent\whilewidth\strut\algorithmicwhile\ #1\ \algorithmicdo\strut}}{\algorithmicend\ \algorithmicwhile}%
\algnewcommand{\parState}[1]{\State%
	\parbox[t]{\dimexpr\linewidth-\algmargin}{\strut #1\strut}}

\makeatletter
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}






\newtheoremrep{thm}{Theorem}[section]
\newtheoremrep{lem}[thm]{Lemma}
\newtheoremrep{pro}[thm]{Proposition}
\newtheoremrep{cor}[thm]{Corollary}
\newtheoremrep{conj}[thm]{Conjecture}
\newtheoremrep{dfn}[thm]{Definition}
\newtheoremrep{exm}[thm]{Example}
\newtheorem{rem}[thm]{Remark}
\newtheoremrep{ass}[thm]{Assumption}
\newtheoremrep{claim}[thm]{Claim}
\newtheoremrep{observation}[thm]{Observation}
\newtheoremrep{counter}[thm]{Counterexample}

\newcommand{\call}{\mathcal{L}}     
\newcommand{\calm}{\mathcal{M}}     
\newcommand{\cals}{\mathcal{S}}     
\newcommand{\caln}{\mathcal{N}}
\newcommand{\calt}{\mathcal{T}}
\newcommand{\calg}{\mathcal{G}}
\newcommand{\cali}{\mathcal{I}}
\newcommand{\cala}{\mathcal{A}}
\newcommand{\calx}{\mathcal{X}}
\newcommand{\calr}{\mathcal{R}}
\newcommand{\calk}{\mathcal{K}}
\newcommand{\cald}{\mathcal{D}}
\newcommand{\calw}{\mathcal{W}}
\newcommand{\calv}{\mathcal{V}}
\newcommand{\cale}{\mathcal{E}}
\newcommand{\calq}{\mathcal{Q}}
\newcommand{\calp}{\mathcal{P}}
\newcommand{\calb}{\mathcal{B}}
\newcommand{\calj}{\mathcal{J}}
\newcommand{\caly}{\mathcal{Y}}

\newcommand{\la}{{\lambda}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bN}{\boldsymbol{N}}
\newcommand{\bA}{\boldsymbol{A}}

\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bq}{\boldsymbol{q}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bc}{\boldsymbol{c}}

\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bla}{\boldsymbol{\lambda}}
\newcommand{\bga}{\boldsymbol{\gamma}}
\newcommand{\bthe}{\bold symbol{\theta}}
\newcommand{\bl}{\boldsymbol{\ell}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\ind}{\boldsymbol{1}}
\newcommand{\bze}{\boldsymbol{\zeta}}
\newcommand{\got}{\textsf{GOT}\xspace}
\newcommand{\ex}{\mathbb{E}}
\newcommand{\pr}{\mathbb{P}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\E}{\mathbb{E}}

\newcommand{\rfok}{\mathsf{RFOK}\xspace}
\newcommand{\gfok}{\mathsf{GFOK}\xspace}
\newcommand{\OPT}{\mathsf{OPT}}
\newcommand{\ECT}{\mathsf{ECT}}
\newcommand{\ECTa}{\mathsf{ECT}[\alpha]}
\newcommand{\LAECT}{\mathsf{LA\text{-}ECT}}
\newcommand{\LAECTg}{\mathsf{LA\text{-}ECT}[\gamma]}
\newcommand{\ALG}{\mathsf{ALG}}
\newcommand{\APX}{\mathsf{APX}}
\newcommand{\ORACLE}{\mathsf{ORACLE}}
\newcommand{\OKP}{\mathsf{OKP}}
\newcommand{\ZCL}{\mathsf{ZCL}}
\newcommand{\ZCLRand}{\mathsf{ZCL\text{-}Randomized}}
\newcommand{\Knapsack}{\mathsf{Knapsack}}
\newcommand{\OTA}{\mathsf{OTA}}


==> laectconst.tex <==
\begin{thmrep}\label{thm:laectConsist}
For any $\mathcal{I} \in \Omega$, let $d_{\max}$ be the highest value density of any item in $\mathcal{I}$, and define $\varrho := d_{\max}/d^\star \geq 1$. Then, for any $\gamma \in (0, 1]$, %
$\LAECTg$ is $\frac{\varrho + 2}{\gamma}$-consistent for accurate predictions.
\end{thmrep}
\begin{proofsketch}
    Assuming the predictions are accurate, the competitive ratio of the algorithm can be analyzed against a semi-online algorithm called $\ORACLE^\star$ (Lemma \ref{lem:oracle}), which we show to be within a constant factor of $\OPT$. The idea is, for a given arbitrary instance $\mathcal{I}$, to compare the utilization and the total value attained for $\mathcal{I}$ between $\ORACLE^\star$ and $\LAECTg$ carefully. If our algorithm terminates within the fair region, we can show that it accepts a superset of what $\ORACLE^\star$ obtains. If our algorithm terminates after the fair region, we can approximate the total value by means of an integral once again, and carry out a similar case analysis as in Theorems \ref{thm:baseline} or \ref{thm:ectComp}.
\end{proofsketch}
\begin{proof}
For consistency, assume that the prediction $\hat{d}$ is accurate (i.e. $\hat{d} = d^\star$).  We first consider how well any algorithm can compete against $\OPT$, given that it knows $d^\star$ exactly.

In Lemma \ref{lem:oracle}, we describe $\ORACLE^\star$, a competitive \textit{semi-online algorithm} \cite{Seiden:00:SemiOnline, Tan:07:SemiOnline, Kumar:19:SemiOnline, Dwibedy:22:SemiOnline}. In other words, it is an algorithm that has full knowledge of the items in the instance, but must process items sequentially using a threshold it has to set in advance.  Items still arrive in an online manner, decisions are immediate and irrevocable, and the order of arrival is unknown.

\begin{lem} \label{lem:oracle}
There is a deterministic semi-online algorithm, $\ORACLE^\star$, which is $1$-CTIF, and has an approximation factor of $2/(1-\epsilon)$, where $\epsilon$ is the upper bound for item weights. Moreover, no deterministic semi-online algorithm with an approximation factor less than $2-L/U$ is $1$-CTIF.
\end{lem}
\paragraph{Proof of Lemma \ref{lem:oracle}} \ \\
\textbf{Upper bound:} 
Recall the definitions of the offline approximation algorithm $\APX$ and optimal threshold $d^\star$ from Definition \ref{dfn:dstar}.  For an arbitrary instance $\mathcal{I}$, let $V$ denote the value obtained by $\APX(\mathcal{I})$, and let $x \in [L,U]$ denote the lowest value density of any item chosen in $\APX(\mathcal{I})$.

Note that $\ORACLE^\star$ can compute $d^\star$ before the items start coming in. So now suppose $\ORACLE^\star$ sets its threshold at $d^\star$, and therefore admits any items with value density above $d^\star$.

There are two cases, listed below. In each case, we show that $\ORACLE^\star$ obtains a value of at least $V/2$:

\begin{itemize}
    \item If $d^\star = x$, we know that the total value of items with value density equal to $x$ in the knapsack of $\APX(\mathcal{I})$ is $V/2$ or larger. Thus, $\ORACLE^\star(\mathcal{I})$ accepts items with value density at least $x$, and the total value of items in the knapsack of $\ORACLE^\star$ will be $V/2$ or larger.
    \item Otherwise, if $d^\star = x^+$ (where $x^+$ is strictly larger than $x$ and strictly smaller than the next density in the sorted order), we know that the total value of items with value density $x$ in the knapsack of $\APX$ is less than $V/2$.  Thus, $\ORACLE^\star(\mathcal{I})$ will reject items of value density $x$, and accept anything with value density larger than $x$, thus obtaining a solution of value at least $V/2$.
\end{itemize}

Therefore, $\ORACLE^\star$ admits a value of at least $V/2$, and its approximation factor is at most $2/(1-\epsilon)$.

\textbf{Lower bound:} Consider an input formed by a large number of infinitesimal items of density $L$ and total weight 1, followed by infinitesimal items of density $U$ and total weight $L/U$. An optimal algorithm accepts all items of density $U$ and fills the remaining space with items of density $L$, giving its knapsack a total value of $(L/U)U + (1-L/U)L = 2L - L^2/U$.
Any deterministic algorithm that satisfies $1$-CTIF, however, must accept either all items of density $L$, giving its knapsack a value of $L$, or reject all items of density $L$, giving it a value of $(L/U)U = L$. In both cases, the approximation factor of the algorithm would be $\frac{2L - L^2/U}{L} = 2-L/U$. \qed

Using $\ORACLE^\star$ as a benchmark, we continue with the proof of Theorem \ref{thm:laectConsist}. Fix an arbitrary input $\mathcal{I} \in \Omega$.  Let $\LAECTg$ terminate filling $z_T$ fraction of the knapsack and obtaining a value of $\LAECTg(\mathcal{I})$.  Let $\ORACLE^\star$ terminate filling $z_O$ fraction of the knapsack and obtaining a value of $\ORACLE^\star(\mathcal{I})$. Denote the maximum possible (offline) value as $\OPT(\mathcal{I})$.

We know that $z_T \geq \kappa$, because $\hat{d}$ is an accurate prediction and thus there exist sufficiently many items in the sequence with value density $\geq \hat{d}$.  Now we consider two cases -- the case where $z_T < \kappa + \gamma$, and the case where $z_T \geq \kappa+\gamma$.  We explore each below.
\paragraph{Case I.} If $z_T < \kappa + \gamma$, the following statements must be true:
\begin{itemize}
    \item $\ORACLE^\star(\mathcal{I})$ does not fill the knapsack.  If it did, $\LAECTg(\mathcal{I})$ would be able to accept additional items such that $z_T \geq \kappa + \gamma$.
    \item It must be the case that $z_O \leq z_T$.  Otherwise, since the threshold function $\Psi^{\gamma, \hat{d}}(z) \leq \hat{d} \forall z \leq \kappa + \gamma$, $\LAECTg(\mathcal{I})$ should have accepted more items such that $z_T \geq z_O$.
    \item if $z_O = z_T$, $\ORACLE^\star(\mathcal{I}) = \LAECTg(\mathcal{I})$, and both algorithms admit the same set of items.  By definition, any item accepted by $\ORACLE^\star(\mathcal{I})$ is accepted by $\LAECTg(\mathcal{I})$.  If any items are accepted by $\LAECTg(\mathcal{I})$ which are not accepted by $\ORACLE^\star(\mathcal{I})$, then it must be the case that $z_T > z_O$.
    \item Furthermore, if $z_O < z_T$, $\ORACLE^\star(\mathcal{I}) < \LAECTg(\mathcal{I})$.  Again, any item accepted by $\ORACLE^\star(\mathcal{I})$ is accepted by $\LAECTg(\mathcal{I})$, and both knapsacks are not full.  Thus, any additional items accepted by $\LAECTg(\mathcal{I})$ add to the total value achieved by $\ORACLE^\star(\mathcal{I})$.
\end{itemize}
Note that \textbf{Case I} implies that as $\gamma$ approaches $1$, the value obtained by $\LAECTg(\mathcal{I})$ is greater than or equal to that obtained by $\ORACLE^\star(\mathcal{I})$, and we inherit the competitive bound of $\ORACLE^\star(\mathcal{I})$ (i.e.,~$\frac{\OPT(\mathcal{I})}{\LAECT[\gamma \rightarrow 1](\mathcal{I})} \leq 2 / (1-\epsilon)$).


\paragraph{Case II.} If $z_T \geq \kappa + \gamma$, we consider two sub-cases based on the definition of $d^\star$.

First, we derive the worst-case value obtained by $\LAECT$.  Denote the items picked by $\LAECT$ by $\mathcal{P}$. 
Note that each item $j$ picked in $\mathcal{P}$ must have value density of at least $\Psi^{\gamma, \hat{d}}(z_j)$, where $z_j$ is the knapsack utilization when that item arrives.  Thus, we have that:
\begin{align}
    \LAECTg(\mathcal{I}) & \geq \sum_{j \in \mathcal{P}}  \Psi^{\gamma, \hat{d}}(z_j) \; w_j.
\end{align}

Based on the assumption that individual item weights are much smaller than $1$, we can substitute for $w_j$ with $\delta z_j := z_{j+1} - z_j$ for all $j$.  This substitution allows us to approximate the summation by an integral. We obtain:
\begin{align*}
    \sum_{j \in \mathcal{S}}  \Psi^{\gamma, \hat{d}}(z_j) \; w_j & \approx \int_{0}^{z_T}  \Psi^{\gamma, \hat{d}}(z) dz = \int_{0}^{z_T-\gamma}  \left(\frac{Ue}{L}\right)^{\frac{z}{1-\gamma}} \left( \frac{L}{e} \right) dz + \int_{\kappa}^{\kappa+\gamma} d^\star \; dz\\
    & \geq d^\star \gamma + \int_{0}^{z_T-\gamma}  \left(\frac{Ue}{L}\right)^{\frac{z}{1-\gamma}} \left( \frac{L}{e} \right) dz\\
    & \geq d^\star \gamma + (1-\gamma) \left(\frac{L}{e} \right) \left[ \frac{\left(\frac{Ue}{L}\right)^{\frac{z}{1-\gamma}}}{\ln (Ue/L)} \right]_{0}^{z_T-\gamma} = d^\star \gamma + (1-\gamma) \frac{\Psi^{\gamma, \hat{d}}(z_T)}{\ln (Ue/L)}. 
\end{align*}

Let $d_{\max}$ denote the largest value density of any item in the sequence $\mathcal{I}$, and note that $\Psi^{\gamma, \hat{d}}(z_T) = d_{\max}$ by definition.  We now consider two different sub-cases based on the definition of $d^\star$ (see Definition \ref{dfn:dstar}) -- the case where $d^\star = x$, and the case where $d^\star = x^+$.  We explore each below.

\begin{itemize}
    \item \textbf{Sub-case II(a):} $d^\star = x$, where $x \in [L, U]$ is the lowest value density of any item packed into the knapsack of $\APX(\mathcal{I})$.  By definition of $\ORACLE^\star$ and $d^\star$, an algorithm which accepts all of the items with value density $d^\star$ in the sequence will be at most $2 / (1-\epsilon)$-competitive against $\OPT(\mathcal{I})$.  Thus, since $\LAECTg(\mathcal{I}) \geq d^\star \gamma + (1 - \gamma) \frac{d_{\max}}{\ln ( Ue/L )}$,  the following holds:
    \begin{align}
    \frac{\OPT(\mathcal{I})}{\LAECTg(\mathcal{I})} \leq \frac{\OPT(\mathcal{I})}{d^\star \gamma + (1 - \gamma) \frac{d_{\max}}{\ln ( Ue/L )}} \leq \frac{\OPT(\mathcal{I})}{d^\star \gamma} \leq \frac{2/ (1-\epsilon)}{\gamma}.
    \end{align}
    \item \textbf{Sub-case II(b):} $d^\star = x^+$, where $x^+ \in [L, U]$ denotes the value density marginally higher than $x$ (lowest value density in the knapsack of $\APX(\mathcal{I})$) but lower than the next highest value density in the list of sorted value densities.  Since $d_{\max}$ is the highest value density for any item in the instance, it is also the largest value density accepted by $\APX(\mathcal{I})$.

    In the worst-case, items arrive in non-decreasing order of value density, so $\LAECTg(\mathcal{I})$ fills $\gamma$ fraction of its knapsack with items of value density exactly equal to $d^\star$.

    Suppose that the next higher value density is $d_{\max}$.  In the worst-case, by definition of $\APX(\mathcal{I})$, the total weight of items with value density $d_{\max}$ is at most $(1 - \gamma)$ (otherwise, $\LAECTg(\mathcal{I})$ will be able to accept some of these higher-valued items in the $\gamma$-CTIF region).  $\OPT(\mathcal{I})$ will accept all of the items in the instance with value densities $d_{\max}$, $d^\star$, and potentially some items with value densities lower than $d^\star$ to fill the rest of the knapsack~--~in the worst-case, $\OPT(\mathcal{I}) \leq d^\star \gamma + d_{\max} ( 1- \gamma)$.  Recalling that $\varrho = d_{\max}/d^\star$, we have the following:

    \begin{align}
    \frac{\OPT(\mathcal{I})}{\LAECTg(\mathcal{I})} \leq \frac{d^\star \gamma + d_{\max} ( 1- \gamma)}{d^\star \gamma + (1 - \gamma) \frac{d_{\max}}{\ln ( Ue/L )}} \leq \frac{d^\star \gamma + d_{\max} ( 1- \gamma)}{d^\star \gamma} \leq \frac{d_{\max}}{d^\star \gamma} = \frac{\varrho}{\gamma} \label{eq:consistCR}
    \end{align}
\end{itemize}

It follows in either case that $\LAECTg$ is $\frac{\varrho + 2}{\gamma}$-consistent for accurate predictions.

In practice, it is often reasonable to assume that $\varrho = d_{\max}/d^\star$ is relatively small, e.g.~$\varrho = O(1)$.  Recall that in sub-case II(b), $d_{\max}$ is the largest value density of any item in the sequence and $d^\star = x^+$.  Observe that $d_{\max}$ and $d^\star$ correspond to the largest and (nearly) smallest value densities accepted into the knapsack of $\APX(\mathcal{I})$, which sorts items by value density in non-increasing order and accepts them greedily in that order.  Thus, if such an assumption holds,  $\LAECTg$ is at most $O \left( \frac{1}{\gamma} \right)$-consistent for accurate predictions.  In \S \ref{sec:experiments}, our experimental results further support this assumption.

It is important, however, to note that in theory, there are simple, artificial counterexamples where this assumption may not hold. For instance, if the $\varrho\approx\frac{U}{L}$, our assumption no longer holds and the consistency bound is no longer meaningful. Notably, under such a counterexample we know that any nontrivial algorithm achieves good empirical competitiveness, as $d^\star \thicksim L$ implies that a knapsack of unit capacity can accept all or nearly all of the items.
\end{proof}

\begin{rem}
For most instances, we assume that $\varrho = O(1)$, implying that $d_{\max} = O(d^\star)$. Whenever this assumption holds, Theorem \ref{thm:laectConsist} implies that $\LAECTg$ is $O (1/\gamma)$-consistent.\\
In \S \ref{sec:experiments}, our experimental results further support this assumption as reasonable in practice.
\end{rem}

